From Standalone LLMs to Integrated Intelligence: A Survey of Compound Al Systems

Compound AI Systems (CAIS) are an emerging paradigm that integrates large language models (LLMs) with external components, including retrievers, agents, tools, and orchestrators, to overcome the limitations of standalone models in tasks requiring memory, reasoning, real-time grounding, and multimodal understanding. These systems enable more capable and context-aware behaviors by composing multiple specialized modules into cohesive workflows. Despite growing adoption in both academia and industry, the CAIS landscape remains fragmented and lacks a unified framework for analysis, taxonomy, and evaluation. In this survey, we define the concept of CAIS, propose a multi-dimensional taxonomy based on component roles and orchestration strategies, and analyze four foundational paradigms: Retrieval-Augmented Generation (RAG), LLM Agents, Multimodal LLMs (MLLMs), and Orchestration. We review representative systems, compare design trade-offs, and summarize evaluation methodologies across these paradigms. Finally, we identify key challenges - including scalability, interoperability, benchmarking, and coordination - and outline promising directions for future research. This survey aims to provide researchers and practitioners with a comprehensive foundation for understanding, developing, and advancing the next generation of system-level artificial intelligence.

==> table/evaluation_metric.tex <==
\renewcommand{\arraystretch}{1.75} % Increase row height
\begin{table}[!htbp]
    \centering
    \caption{Summary of Evaluation Dimensions, Benchmarks, and Metrics for Compound AI Systems}
    \resizebox{\textwidth}{!}
    {
    \begin{tabular}{p{2.5cm} p{2.5cm} p{5cm} p{4.5cm}}
        \toprule
        \textbf{Dimension} & \textbf{Task} & \textbf{Datasets/Benchmarks} & \textbf{Evaluation Metrics} \\
        \midrule
        % RAG PART
        \multirow{7}{*}{RAG} 
        & Open-domain QA & \makecell[l]{Natural Questions \cite{kwiatkowski2019natural}, TriviaQA \cite{joshi2017triviaqa}, \\ WebQuestions \cite{berant2013semantic}, RealTimeQA \cite{kasai2023realtime}} & Accuracy, F1 Score, EM \\[0.5ex]
        & Passage Retrieval & MS MARCO \cite{bajaj2016ms}, BEIR \cite{thakur2021beir}, TREC-DL \cite{craswell2021trec} & MRR, nDCG, Precision, Recall, F1 Score \\[0.5ex]
        & Knowledge QA & OpenBookQA \cite{mihaylov2018can}, PopQA \cite{mallen2022not}, TruthfulQA \cite{lin2021truthfulqa} & Accuracy, F1 Score, EM \\[0.5ex]
        & Multi-hop QA & \makecell[l]{HotpotQA \cite{yang2018hotpotqa}, 2WikiMultihopQA \cite{ho2020constructing}, \\ MuSiQue \cite{trivedi2022musique}, StrategyQA \cite{geva2021did}} & EM, F1 Score, Accuracy \\[0.5ex]
        & Extractive QA & SQuAD \cite{rajpurkar2016squad}, DROP \cite{dua2019drop} & EM, F1 Score, Precision, Recall \\[0.5ex]
        & Summarization / Long-form Eval. & \makecell[l]{WikiAsp \cite{hayashi2021wikiasp}, Multi-News \cite{fabbri2019multi}, \\ NarrativeQA \cite{kovcisky2018narrativeqa}, UniEval \cite{zhong2022towards}} & ROUGE, BLEU, F1 Score \\[0.5ex]
        & RAG Pipeline Evaluation & Ragas \cite{es2024ragas}, KILT \cite{petroni2020kilt} & Faithfulness, Context Precision, Context Recall, EM, F1 Score \\
        \midrule
        % Multimodal part
        \multirow{4}{*}{Multimodal LLM} 
        & Reasoning and Commonsense QA & MM-Vet \cite{yu2023mm}, ALLaVA \cite{chen2024allava}, SEED-Bench \cite{li2023seed} & Accuracy, F1 Score, EM, Perplexity \\[0.5ex]
        & Chart and Document Understanding & ChartQA \cite{masry2022chartqa}, MMC-Benchmark \cite{liu2023mmc}, DocVQA \cite{mathew2021docvqa}, TextVQA \cite{singh2019towards} & Accuracy, F1 Score, BLEU, ROUGE \\[0.5ex]
        & Safety and Alignment & MM-SafetyBench \cite{liu2024mm} & Accuracy, F1 Score, Custom Safety Metrics 
        % (e.g., bias, toxicity) 
        \\[0.5ex]
        & Multimodal Evaluation & MME \cite{fu2023mme}, MultiBench \cite{liang2021multibench} & Accuracy, F1 Score, MRR, Perplexity, BLEU, ROUGE \\
        \midrule
         
        % Orchestration part
        \multirow{3}{*}{\makecell[l]{Orchestration of\\ Compound AI \\ Systems}} 
        & Structural Layer & \makecell[l]{BigDataBench \cite{gao2018bigdatabench}, \\ AIBench Training \cite{tang2021aibench}} & Throughput, Latency Overhead, Bandwidth Utilization  \\[0.5ex]
        & Mechanism Layer & AISBench \cite{dong2025aisbench}, WebArena \cite{zhou2023webarena}, Long Range Arena \cite{tay2020long}, ZeroSCROLLS \cite{shaham2023zeroscrolls} & Mean Task Completion Time, Average API Response Time, Cache Hit Rate \\[0.5ex]
        & Objective Layer & AI Fairness 360 \cite{bellamy2019ai} &  Fairness-specific metrics\\ 
        \midrule
        % agent part
        \multirow{3}{*}{LLM Agents} 
        & Role-Playing  & RoleLLM \cite{wang2023rolellm}, AgentBench \cite{liu2023agentbench} , AgentBoard \cite{ma2024agentboard} &
        Role-Consistency Score, Self-Correction Rate
        \\[0.5ex]
        & Interactive Reasoning & AgentQuest \cite{gioacchini2024agentquest}, InfiAgent-DABench \cite{hu2024infiagent}, CriticBench \cite{lin2024criticbench} & 
        Reasoning Trace Accuracy, Generalization Score
        \\[0.5ex]
        & Tool Use & 
        ML-Bench \cite{tang2023ml}, Berkeley Function Calling Leaderboard \cite{berkeley-function-calling-leaderboard} &
        Tool Call Accuracy, Token Efficiency
        \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:evaluation_frameworks}
\end{table}
